Localization Coverage Analysis of THz Communication Systems with a 3D Array

This paper considers the problem of estimating the position and orientation of a user equipped with a three-dimensional (3D) array receiving downlink far-field THz signals from multiple base stations with known positions and orientations. We derive the Cram\'er-Rao Bound for the localization problem and define the coverage of the considered system. We compare the error lower bound distributions of the conventional planar array and the 3D array configurations at different user equipment (UE) positions and orientations. Our numerical results obtained for array configurations with an equal number of elements show very limited coverage of the planar-array configuration, especially across the UE orientation range. Conversely, a 3D array configuration offers an overall higher coverage with minor performance loss in certain UE positions and orientations.

==> main_0413 2/Acronyms.tex <==
% \newlist{acronyms}{description}{1}
% \setlist[acronyms]{
% labelwidth = 4.5em,
% leftmargin = 5em,
% noitemsep,
% itemindent = 0pt}
% \DeclareAcroListStyle{mystyle}{list}{ list = acronyms }
% \acsetup{ list-style = mystyle }

\DeclareAcronym{5g}{
short=5G,
long= fifth generation,
}
\DeclareAcronym{6g}{
short=6G,
long= sixth generation,
}
\DeclareAcronym{3d}{
short=3D,
long= three-dimensional,
}
\DeclareAcronym{2d}{
short=2D,
long= two-dimensional,
}
\DeclareAcronym{aod}{
short=AOD,
long= angle-of-departure,
}
\DeclareAcronym{aosa}{
short=AOSA,
long= array-of-subarray,
}
\DeclareAcronym{adod}{
short=ADOD,
long= angle-difference-of-departure,
}
\DeclareAcronym{aoa}{
short=AOA,
long= angle-of-arrival,
}
\DeclareAcronym{adc}{
short=ADC,
long= analog to digital converter,
}
\DeclareAcronym{aeb}{
short=AEB,
long= angle error bound,
}
\DeclareAcronym{av}{
short=AV,
long= autonomous vehicle,
}
\DeclareAcronym{bs}{
short=BS,
long= base station,
}

\DeclareAcronym{csi}{
short=CSI,
long= channel state information,
}
\DeclareAcronym{cfo}{
short=CFO,
long= carrier frequency offset,
}
\DeclareAcronym{ceb}{
short=CEB,
long= clock error bound,
}
\DeclareAcronym{coa}{
short=COA,
long= curvature-of-arrival,
}
\DeclareAcronym{crb}{
short=CRB,
long= Cram\'er-Rao bound,
}
\DeclareAcronym{ccrb}{
short=CCRB,
long= constrained Cram\'er-Rao bound,
}
\DeclareAcronym{cmos}{
short=CMOS,
long= complementary metal-oxide-semiconductor,
}
\DeclareAcronym{crlb}{
short=CRLB,
long= Cram\'er-Rao lower bound,
}
\DeclareAcronym{cdf}{
short=CDF,
long= cumulative distribution function,
}
\DeclareAcronym{cp}{
short=CP,
long= cyclic prefix,
}
\DeclareAcronym{dac}{
short=DAC,
long= digital to analog converter,
}
\DeclareAcronym{dfl}{
short=DFL,
long= device-free localization,
}
\DeclareAcronym{dmimo}{
short=D-MIMO,
long= distributed MIMO,
}
\DeclareAcronym{dlprs}{
short=DL-PRS,
long= downlink positioning reference signal,
}
\DeclareAcronym{d2d}{
short=D2D,
long= device-to-device,
}
\DeclareAcronym{dftsofdm}{
short=DFT-s-OFDM,
long= discrete-Fourier-transform spread OFDM,
}
\DeclareAcronym{dl}{
short=DL,
long= deep learning,
}
\DeclareAcronym{gps}{
short=GPS,
long= global positioning system,
}
\DeclareAcronym{gnss}{
short=GNSS,
long= global navigation satellite system,
}
\DeclareAcronym{fim}{
short=FIM,
long = Fisher information matrix,
}
\DeclareAcronym{hwi}{
short=HWI,
long= hardware impairment,
}
\DeclareAcronym{hemt}{
short=HEMT,
long= high electron mobility transistor,
}
\DeclareAcronym{hbt}{
short=HBT,
long= heterojunction bipolar transistors,
}
\DeclareAcronym{iot}{
short=IoT,
long= internet of things,
}
\DeclareAcronym{imu}{
short=IMU,
long= inertial measurement unit,
}
\DeclareAcronym{isac}{
short=ISAC,
long= integrated sensing and communication,
}
\DeclareAcronym{iqi}{
short=IQI,
long= in-phase and quadrature imbalance,
}
\DeclareAcronym{ip}{
short=IP,
long= incidence point,
}
\DeclareAcronym{ia}{
short=IA,
long= initial access,
}
\DeclareAcronym{kpi}{
short=KPI,
long= key performance indicator,
}
\DeclareAcronym{kf}{
short=KF,
long= Kalman filter,
}
\DeclareAcronym{ekf}{
short=EKF,
long= extended Kalman filter,
}
\DeclareAcronym{ukf}{
short=UKF,
long= unscented Kalman filter,
}
\DeclareAcronym{ckf}{
short=CKF,
long= cubature Kalman filter,
}
\DeclareAcronym{pf}{
short=PF,
long= particle filter,
}
\DeclareAcronym{lb}{
short=LB,
long= lower bound,
}
\DeclareAcronym{lse}{
short=LSE,
long= least-square estimator,
}
\DeclareAcronym{lo}{
short=LO,
long= local oscillator,
}
\DeclareAcronym{los}{
short=LOS,
long= line-of-sight,
}
\DeclareAcronym{mc}{
short=MC,
long= mutual coupling,
}
\DeclareAcronym{mac}{
short=MAC,
long= medium access control,
}
\DeclareAcronym{meb}{
short=MEB,
long= mapping error bound,
}
\DeclareAcronym{ml}{
short=ML,
long= machine learning,
}
\DeclareAcronym{mcrb}{
short=MCRB,
long= misspecified Cram\'er-Rao bound,
}
\DeclareAcronym{mds}{
short=MDS,
long= multidimensional scaling ,
}
\DeclareAcronym{mimo}{
short=MIMO,
long= multiple-input-multiple-output,
}
\DeclareAcronym{siso}{
short=SISO,
long= single-input-single-output,
}
\DeclareAcronym{mm}{
short=MM,
long= mismatched model,
}
\DeclareAcronym{mpc}{
short=MPC,
long= multipath components,
}
\DeclareAcronym{mmwave}{
short=mmWave,
long= millimeter wave,
}
\DeclareAcronym{mmle}{
short=MMLE,
long= mismatched maximum likelihood estimation,
}
\DeclareAcronym{mems}{
short=MEMS,
long= micro-electro-mechanical system,
}
\DeclareAcronym{mle}{
short=MLE,
long= maximum likelihood estimation,
}
\DeclareAcronym{nlos}{
short=NLOS,
long= none-line-of-sight,
}
\DeclareAcronym{ofdm}{
short=OFDM,
long= orthogonal frequency-division multiplexing,
}
\DeclareAcronym{oeb}{
short=OEB,
long= orientation error bound,
}
\DeclareAcronym{otfs}{
short=OTFS,
long= orthogonal time-frequency space,
}
\DeclareAcronym{pdf}{
short=PDF,
long= probability density function,
}
\DeclareAcronym{papr}{
short=PAPR,
long= peak-to-average-power ratio,
}
\DeclareAcronym{pan}{
short=PAN,
long= power amplifier nonlinearity,
}
\DeclareAcronym{pa}{
short=PA,
long= power amplifier,
}
\DeclareAcronym{ps}{
short=PS,
long= phase shifter,
}
\DeclareAcronym{pn}{
short=PN,
long= phase noise,
}
\DeclareAcronym{poa}{
short=POA,
long= phase-of-arrival,
}
\DeclareAcronym{pwm}{
short=PWM,
long= planar wave model,
}
\DeclareAcronym{pdoa}{
short=PDOA,
long= phase-difference-of-arrival,
}
\DeclareAcronym{prs}{
short=PRS,
long= positioning reference signals,
}
\DeclareAcronym{peb}{
short=PEB,
long= position error bound,
}
\DeclareAcronym{rnn}{
short=RNN,
long= recurrent neural network,
}
\DeclareAcronym{rl}{
short=RL,
long= reinforcement learning,
}
\DeclareAcronym{rfc}{
short=RFC,
long= radio-frequency chain,
}
\DeclareAcronym{rf}{
short=RF,
long= radio frequency,
}
\DeclareAcronym{rfid}{
short=RFID,
long= radio frequency identification,
}
\DeclareAcronym{ris}{
short=RIS,
long= reconfigurable intelligent surface,
}
\DeclareAcronym{rss}{
short=RSS,
long= received signal strength,
}
\DeclareAcronym{rtt}{
short=RTT,
long= round-trip time,
}
\DeclareAcronym{sm}{
short=SM,
long= standard model,
}
\DeclareAcronym{sige}{
short=SiGe,
long= silicon-germanium,
}
\DeclareAcronym{spp}{
short=SPP,
long= surface plasmon polariton,
}
\DeclareAcronym{sa}{
short=SA,
long= subarray,
}
\DeclareAcronym{sota}{
short=SOTA,
long= state-of-the-art,
}
\DeclareAcronym{swm}{
short=SWM,
long= spherical wave model,
}
\DeclareAcronym{slam}{
short=SLAM,
long= simultaneous localization and mapping,
}
\DeclareAcronym{tm}{
short=TM,
long= true model,
}
\DeclareAcronym{toa}{
short=TOA,
long= time-of-arrival,
}
\DeclareAcronym{tof}{
short=TOF,
long= time-of-flight,
}
\DeclareAcronym{tdoa}{
short=TDOA,
long= time-difference-of-arrival,
}
\DeclareAcronym{thz}{
short=THz,
long= Terahertz,
}
\DeclareAcronym{ue}{
short=UE,
long= user equipment,
}
\DeclareAcronym{ummimo}{
short=UM-MIMO,
long= ultra-massive multi-input-multi-output,
}
\DeclareAcronym{vlp}{
short=VLP,
long= visible light positioning,
}
\DeclareAcronym{veb}{
short=VEB,
long= velocity error bound,
}
\DeclareAcronym{vlc}{
short=VLC,
long= visible light communication,
}
\DeclareAcronym{ula}{
short=ULA,
long= uniform linear array,
}
\DeclareAcronym{uav}{
short=UAV,
long= unmanned aerial vehicle,
}
\DeclareAcronym{upa}{
short=UPA,
long= uniform planar array,
}
\DeclareAcronym{wlan}{
short=WLAN,
long= wireless local area network,
}



























==> main_0413 2/fig-6-1.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,1.00000,1.00000}%
\begin{tikzpicture}
[scale=1\columnwidth/10cm,font=\normalsize]
\begin{axis}[%
width=9cm,
height=3cm,
at={(0,0)},
scale only axis,
xmode=log,
xmin=0.001,
xmax=200,
xminorticks=true,
xticklabel style = {font=\tiny,yshift=0.5ex},
xlabel style={font=\footnotesize\color{white!15!black}, yshift=1 ex},
xlabel={PEB threshold $\xi_p$ [m]},
ymode=log,
ymin=0.001,
ymax=1,
yminorticks=true,
yticklabel style = {font=\tiny,xshift=0.5ex},
ylabel style={font=\footnotesize\color{white!15!black}, yshift= -1.5 ex},
ylabel={$1-C_p(\xi_p)$},
axis background/.style={fill=white},
xmajorgrids,
% xminorgrids,
ymajorgrids,
% yminorgrids,
% legend style={legend cell align=left, align=left, draw=white!15!black}
legend style={font=\scriptsize, at={(.02, 0.02)}, anchor=south west, legend cell align=left, align=left, draw=white!5!black, legend columns=1}
]
\addplot [color=red, dashed, line width=1.0pt]
  table[row sep=crcr]{%
0.00321377485631557	1\\
0.00517543224182616	0.9993\\
0.00781542030119936	0.998\\
0.0124487691356384	0.9956\\
0.0186705669039656	0.9904\\
0.0279501778688199	0.9848\\
0.0417185901223784	0.978\\
0.062321209447348	0.9705\\
0.093707551494477	0.959800000000001\\
0.139852152561469	0.945700000000001\\
0.20883273957495	0.922700000000002\\
0.311811179961362	0.904700000000003\\
0.46683163964723	0.891100000000004\\
0.696621721634031	0.881700000000004\\
1.05117919455885	0.871400000000005\\
1.57558396258669	0.858400000000006\\
2.35262132556694	0.842800000000007\\
3.52145848398286	0.822900000000009\\
5.25955457176439	0.794800000000011\\
7.8535305894718	0.756800000000015\\
11.7210760013371	0.70530000000002\\
17.4868211046102	0.639600000000028\\
26.0893073805547	0.559000000000037\\
38.932998618345	0.45940000000004\\
58.0818149604605	0.333200000000031\\
83.1522339945544	0.223300000000024\\
112.838583380745	0.149600000000014\\
169.15443716115	0.107800000000009\\
272.684897474049	0.105000000000009\\
425.278655724301	0.104700000000009\\
648.305865406137	0.104500000000009\\
1164.31170296725	0.104300000000009\\
1607.61228191207	0.104200000000009\\
};
\addlegendentry{2 BSs (Planar)}

\addplot [color=red, line width=1.0pt]
  table[row sep=crcr]{%
0.00394519859895781	1\\
0.00591148549096145	0.9984\\
0.00883800368513104	0.9947\\
0.0132007173727278	0.9847\\
0.0198066407956929	0.966800000000001\\
0.0295695680150252	0.941400000000001\\
0.0441969867078869	0.905400000000003\\
0.0660101104768214	0.853500000000006\\
0.0985692647069242	0.775700000000013\\
0.147074994597406	0.649000000000027\\
0.219410175127795	0.464000000000041\\
0.327360329092341	0.323100000000031\\
0.475280604005696	0.216500000000023\\
0.687822867618061	0.145100000000014\\
1.02553364873781	0.0972000000000083\\
1.51608122698459	0.0651000000000058\\
2.2142035086038	0.0436000000000039\\
3.05408283025137	0.0292000000000024\\
4.25101442879755	0.0195000000000016\\
6.28562293103789	0.0130000000000011\\
8.37527667044991	0.00870000000000071\\
10.6790561635095	0.00580000000000047\\
13.2263929790069	0.00380000000000036\\
16.7638009166723	0.00250000000000017\\
21.0375904341182	0.00160000000000016\\
32.0145368513233	0.00100000000000011\\
35.504002365593	0.000600000000000045\\
37.9607947010018	0.000400000000000067\\
45.1064238958506	0.000199999999999978\\
49.3786550015562	9.9999999999989e-05\\
62.6339317785765	0\\
};
\addlegendentry{2 BSs (Cuboidal)}

\addplot [color=mycolor1, dashed, line width=1.0pt]
  table[row sep=crcr]{%
0.00224122868896719	1\\
0.00362677558045581	0.9989\\
0.00542663136118943	0.9961\\
0.00819226415972954	0.9913\\
0.0122225469865515	0.98\\
0.0182669824811898	0.969\\
0.0272822552301265	0.949700000000001\\
0.0407484026470011	0.924200000000002\\
0.0608356197849411	0.885500000000004\\
0.0908739055284702	0.837600000000007\\
0.135884801588524	0.784600000000012\\
0.202818365117429	0.732800000000017\\
0.303083586154082	0.678700000000023\\
0.452156547373415	0.62220000000003\\
0.6752382586051	0.575100000000035\\
1.00992450384714	0.545500000000038\\
1.50815871543884	0.519200000000041\\
2.25455959343592	0.499000000000043\\
3.36473292828412	0.481600000000042\\
5.06226949555169	0.46110000000004\\
7.56132571839429	0.436800000000038\\
11.298421165133	0.406900000000036\\
16.8626711454129	0.373300000000033\\
25.1608385979553	0.331600000000031\\
37.5393991994462	0.283400000000029\\
56.0812164064648	0.221000000000024\\
83.7765802492176	0.161100000000016\\
125.453257648085	0.11850000000001\\
192.797686056502	0.105400000000009\\
295.052694722384	0.104600000000009\\
648.305865406137	0.104400000000009\\
1164.31170296725	0.104200000000009\\
1164.31170296725	0.104200000000009\\
};
\addlegendentry{3 BSs (Planar)}

\addplot [color=mycolor1, line width=1.0pt]
  table[row sep=crcr]{%
0.00224373808957186	1\\
0.00347916047567224	0.9986\\
0.00520558495488861	0.9962\\
0.00784040936270329	0.991\\
0.011753164233544	0.9755\\
0.0175746375137446	0.946800000000001\\
0.0262190615901001	0.909200000000003\\
0.0391580252135708	0.849400000000006\\
0.0584665851991121	0.746900000000016\\
0.0872261868288971	0.541300000000039\\
0.124252167644244	0.362800000000032\\
0.162828645425025	0.243100000000027\\
0.209255463960246	0.162900000000016\\
0.259793274537583	0.109100000000009\\
0.308561269466112	0.0731000000000064\\
0.363346860006002	0.0490000000000044\\
0.418619248782518	0.0328000000000028\\
0.468732474855943	0.0219000000000018\\
0.51823614006173	0.0146000000000012\\
0.567563018193133	0.00970000000000082\\
0.626617878009936	0.00650000000000051\\
0.681233649915063	0.00430000000000041\\
0.705945496485931	0.00280000000000025\\
0.732395557092933	0.00180000000000013\\
0.765499703331553	0.00120000000000009\\
0.789319083689008	0.000800000000000023\\
0.812490330983125	0.000500000000000056\\
0.847407790462	0.000300000000000078\\
0.860331596063971	0.000199999999999978\\
0.877816740553667	9.9999999999989e-05\\
0.878020827721896	0\\
};
\addlegendentry{3 BSs (Cuboidal)}

\addplot [color=blue, dashdotted, line width=1.0pt]
  table[row sep=crcr]{%
0.00226598406059725	1\\
0.00346644074995861	0.9986\\
0.00536023690436872	0.9943\\
0.00803489033883614	0.9852\\
0.0119952251932998	0.9707\\
0.0178974714335381	0.948600000000001\\
0.0267152999139203	0.920200000000002\\
0.039892796773114	0.878500000000004\\
0.0596652749102274	0.817000000000009\\
0.0890230778198991	0.727500000000018\\
0.132844227163463	0.640300000000028\\
0.198189569590311	0.557100000000037\\
0.295883406304848	0.467800000000041\\
0.441415533831599	0.375700000000033\\
0.6589621217252	0.289500000000029\\
0.983753547950755	0.228200000000025\\
1.46851536335774	0.18900000000002\\
2.19090552041143	0.162400000000016\\
3.27964406967947	0.144200000000013\\
4.90415811600568	0.133200000000012\\
7.3804881187431	0.124200000000011\\
11.0184833931092	0.11760000000001\\
16.4758815805257	0.11430000000001\\
24.6426076265896	0.110900000000009\\
37.3538015900475	0.109200000000009\\
63.911805741808	0.107700000000009\\
118.247710007735	0.107400000000009\\
397.418680629925	0.107300000000009\\
397.418680629925	0.107300000000009\\
};
\addlegendentry{4 BSs (Planar)}

\addplot [color=blue, line width=1.0pt]
  table[row sep=crcr]{%
0.00203190853962711	1\\
0.00306921807879053	0.9994\\
0.00460299288262007	0.9954\\
0.00687630174873875	0.9878\\
0.0102624329471492	0.9709\\
0.0153126501708556	0.935600000000001\\
0.0228685675875398	0.883500000000004\\
0.0341305457610686	0.809000000000009\\
0.0509203763918155	0.670200000000024\\
0.0670182252224179	0.449200000000039\\
0.0770539071971637	0.301100000000029\\
0.0858918481919814	0.201800000000022\\
0.0918994870832602	0.135200000000012\\
0.0964803495330317	0.0906000000000078\\
0.0999415113268414	0.0607000000000054\\
0.102832297793057	0.0406000000000035\\
0.104786829983194	0.0272000000000023\\
0.106598766214251	0.0182000000000015\\
0.108082290436103	0.012100000000001\\
0.109263887583457	0.00810000000000066\\
0.110897289666588	0.00540000000000052\\
0.112834814346186	0.00360000000000027\\
0.113700825837012	0.00240000000000018\\
0.116703734386609	0.00160000000000016\\
0.12124962392021	0.00100000000000011\\
0.12406332873144	0.000600000000000045\\
0.124662532147836	0.000400000000000067\\
0.131851752698005	0.000199999999999978\\
0.132085552903972	9.9999999999989e-05\\
0.135269190286375	0\\
};
\addlegendentry{4 BSs (Cuboidal)}

\end{axis}
% \begin{axis}[%
% width=7.778in,
% height=5.833in,
% at={(0in,0in)},
% scale only axis,
% xmin=0,
% xmax=1,
% ymin=0,
% ymax=1,
% axis line style={draw=none},
% ticks=none,
% axis x line*=bottom,
% axis y line*=left
% ]
% \end{axis}
\end{tikzpicture}%

==> main_0413 2/fig-6-2.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,1.00000,1.00000}%
\begin{tikzpicture}
[scale=1\columnwidth/10cm,font=\normalsize]
\begin{axis}[%
width=9cm,
height=3cm,
at={(0,0)},
scale only axis,
xmode=log,
xmin=0.0005,
xmax=50,
xminorticks=true,
xticklabel style = {font=\tiny,yshift=0.5ex},
xlabel style={font=\footnotesize\color{white!15!black}, yshift=1 ex},
xlabel={OEB threshold $\xi_o$ [deg]},
ymode=log,
ymin=0.001,
ymax=1,
yminorticks=true,
yticklabel style = {font=\tiny,xshift=0.5ex},
ylabel style={font=\footnotesize\color{white!15!black}, yshift= -1.5 ex},
ylabel={$1-C_o(\xi_o)$},
axis background/.style={fill=white},
xmajorgrids,
% xminorgrids,
ymajorgrids,
% yminorgrids,
% legend style={legend cell align=left, align=left, draw=white!15!black}
legend style={font=\scriptsize, at={(.02, 0.02)}, anchor=south west, legend cell align=left, align=left, draw=white!5!black, legend columns=1}
]
\addplot [color=red, dashed, line width=1.0pt]
  table[row sep=crcr]{%
0.00988787744279652	1\\
0.0185295347239062	0.9997\\
0.0276591561985474	0.9932\\
0.0412688629656109	0.9675\\
0.0616765415399533	0.931900000000002\\
0.0923384347062284	0.906900000000003\\
0.13808540797836	0.891700000000004\\
0.206665210526993	0.882200000000004\\
0.309412821709501	0.869300000000005\\
0.461906374493165	0.850800000000006\\
0.689228783624722	0.823000000000009\\
1.03002654343277	0.779800000000012\\
1.53675329895479	0.71150000000002\\
2.29292420564922	0.62000000000003\\
3.42141112372871	0.485400000000042\\
5.10709269179051	0.334400000000031\\
7.62095660845797	0.235800000000026\\
11.3856855225076	0.179100000000019\\
16.9902396070313	0.146100000000014\\
25.5563276237848	0.127700000000011\\
38.3092748692102	0.11770000000001\\
57.3257091584356	0.11380000000001\\
85.882217195609	0.111800000000009\\
130.732455031087	0.110800000000009\\
222.566101298458	0.110400000000009\\
356.859867829975	0.109700000000009\\
532.701598173601	0.109000000000009\\
876.916138847247	0.108300000000009\\
1371.30436828515	0.107100000000009\\
2096.16390093305	0.105800000000009\\
3765.38016074861	0.105300000000009\\
6512.42135994069	0.104700000000009\\
9512.67624410014	0.104200000000009\\
};
\addlegendentry{2 BSs (Planar)}

\addplot [color=red, line width=1.0pt]
  table[row sep=crcr]{%
0.0208274477548481	1\\
0.032493592311319	0.9995\\
0.0484838936343419	0.892200000000004\\
0.0619416141552267	0.598000000000032\\
0.0815062144110277	0.400800000000035\\
0.112166151741289	0.268600000000028\\
0.161950166564783	0.180000000000019\\
0.235176992165153	0.12060000000001\\
0.346305168262226	0.0808000000000071\\
0.499467491554229	0.0541000000000048\\
0.699098773048834	0.0362000000000031\\
1.00888696057339	0.024200000000002\\
1.38527879758983	0.0162000000000013\\
1.76659389288995	0.0108000000000009\\
2.18821791197577	0.00720000000000065\\
3.17378314328166	0.00480000000000036\\
3.84838610647981	0.00320000000000031\\
4.63076580693112	0.00210000000000021\\
4.94333992518417	0.00140000000000007\\
5.39101291754477	0.000900000000000123\\
5.92869372187185	0.000600000000000045\\
6.3731775954022	0.000400000000000067\\
6.75455454164477	0.000199999999999978\\
6.78055679256805	9.9999999999989e-05\\
7.1523249464564	0\\
};
\addlegendentry{2 BSs (Cuboidal)}

\addplot [color=mycolor1, dashed, line width=1.0pt]
  table[row sep=crcr]{%
0.00988787744279652	1\\
0.0147659769258238	0.9978\\
0.0220336839843318	0.958200000000001\\
0.0328848812586802	0.859400000000006\\
0.0490605146392865	0.749000000000016\\
0.0732437805037895	0.657200000000026\\
0.109513830541538	0.598400000000032\\
0.163421939630106	0.559100000000037\\
0.243848648061209	0.534800000000039\\
0.365049216435302	0.509700000000042\\
0.545725749292337	0.487900000000042\\
0.8143472331335	0.463700000000041\\
1.21561860667267	0.431500000000038\\
1.81406904827302	0.387600000000034\\
2.70640325416786	0.331600000000031\\
4.03841119370907	0.259800000000028\\
6.02683897852692	0.195700000000021\\
9.01053942568293	0.158000000000015\\
13.4727787253908	0.134400000000012\\
20.121121694598	0.12260000000001\\
30.1509076119885	0.11440000000001\\
45.5684987632414	0.110000000000009\\
68.5100627049083	0.108900000000009\\
104.48318477729	0.108100000000009\\
259.035307503632	0.107600000000009\\
409.892767266945	0.107100000000009\\
678.947619045273	0.106700000000009\\
1017.92313633972	0.106000000000009\\
1522.98346931693	0.105700000000009\\
4320.1127114385	0.105000000000009\\
6512.42135994069	0.104700000000009\\
9512.67624410014	0.104200000000009\\
};
\addlegendentry{3 BSs (Planar)}

\addplot [color=mycolor1, line width=1.0pt]
  table[row sep=crcr]{%
0.0124894173642895	1\\
0.0191153904492414	0.9992\\
0.0280236212267777	0.669700000000024\\
0.0320612628600523	0.448900000000039\\
0.0361262971854822	0.300900000000029\\
0.040020652411007	0.201600000000022\\
0.0437359410920901	0.135100000000012\\
0.047298663040945	0.0905000000000078\\
0.0512767848323483	0.0606000000000054\\
0.0550236261307899	0.0406000000000035\\
0.0591254274768609	0.0272000000000023\\
0.0624018822887527	0.0182000000000015\\
0.0656692138947683	0.012100000000001\\
0.0687157150345736	0.00810000000000066\\
0.0719508195419081	0.00540000000000052\\
0.074757559326625	0.00360000000000027\\
0.0763385074122478	0.00240000000000018\\
0.0779609308104053	0.00160000000000016\\
0.0797930482355357	0.00100000000000011\\
0.0855268870973913	0.000600000000000045\\
0.0871855691864493	0.000400000000000067\\
0.0872069966504657	0.000199999999999978\\
0.088612366940436	9.9999999999989e-05\\
0.0913141758777622	0\\
};
\addlegendentry{3 BSs (Cuboidal)}

\addplot [color=blue, dashdotted, line width=1.0pt]
  table[row sep=crcr]{%
0.00900010743584662	1\\
0.013561310690623	0.9963\\
0.0202435643439805	0.945900000000001\\
0.0302160579408396	0.790500000000011\\
0.0450807038820125	0.604700000000032\\
0.0672771949072797	0.438100000000038\\
0.100407892348784	0.329400000000031\\
0.1499097151116	0.253100000000028\\
0.223665490225824	0.202300000000022\\
0.333806853578296	0.169200000000017\\
0.498555296954324	0.147700000000014\\
0.751198448971513	0.133200000000012\\
1.12219704249745	0.123400000000011\\
1.6894623471922	0.11750000000001\\
2.53111158794127	0.11290000000001\\
3.79967988681564	0.110100000000009\\
5.85494427629401	0.108600000000009\\
9.20399491839167	0.107800000000009\\
13.8586050511356	0.107700000000009\\
31.1228958372541	0.107400000000009\\
53.147851890805	0.107300000000009\\
53.147851890805	0.107300000000009\\
};
\addlegendentry{4 BSs (Planar)}

\addplot [color=blue, line width=1.0pt]
  table[row sep=crcr]{%
0.0115416281414167	1\\
0.0173674398569388	0.9993\\
0.0224628799202051	0.669800000000024\\
0.0232622990309393	0.448900000000039\\
0.0237894761028864	0.300900000000029\\
0.0242407637428908	0.201600000000022\\
0.0247195986168492	0.135100000000012\\
0.0253089601323678	0.0905000000000078\\
0.0259254684603623	0.0606000000000054\\
0.0265070521978093	0.0406000000000035\\
0.0270881864899894	0.0272000000000023\\
0.0275925554291666	0.0182000000000015\\
0.0282168883957473	0.012100000000001\\
0.0287187740680756	0.00810000000000066\\
0.0291721070451533	0.00540000000000052\\
0.029682807829483	0.00360000000000027\\
0.0303562421590723	0.00240000000000018\\
0.0308081562099251	0.00160000000000016\\
0.031522618485242	0.00100000000000011\\
0.0322200474973032	0.000600000000000045\\
0.0325912180708779	0.000400000000000067\\
0.0340906914933193	0.000199999999999978\\
0.0352395995062225	9.9999999999989e-05\\
0.0368157402029504	0\\
};
\addlegendentry{4 BSs (Cuboidal)}

\end{axis}
% \begin{axis}[%
% width=7.778in,
% height=5.833in,
% at={(0in,0in)},
% scale only axis,
% xmin=0,
% xmax=1,
% ymin=0,
% ymax=1,
% axis line style={draw=none},
% ticks=none,
% axis x line*=bottom,
% axis y line*=left
% ]
% \end{axis}
\end{tikzpicture}%
